Mobile-Cloud Inference for Collaborative Intelligence

As AI applications for mobile devices become more prevalent, there is an increasing need for faster execution and lower energy consumption for deep learning model inference. Historically, the models run on mobile devices have been smaller and simpler in comparison to large state-of-the-art research models, which can only run on the cloud. However, cloud-only inference has drawbacks such as increased network bandwidth consumption and higher latency. In addition, cloud-only inference requires the input data (images, audio) to be fully transferred to the cloud, creating concerns about potential privacy breaches. There is an alternative approach: shared mobile-cloud inference. Partial inference is performed on the mobile in order to reduce the dimensionality of the input data and arrive at a compact feature tensor, which is a latent space representation of the input signal. The feature tensor is then transmitted to the server for further inference. This strategy can reduce inference latency, energy consumption, and network bandwidth usage, as well as provide privacy protection, because the original signal never leaves the mobile. Further performance gain can be achieved by compressing the feature tensor before its transmission.

==> tex/figures/layer_histogram.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{img/misc/layer_histogram.png}
  \caption[Layer output histogram]{%
    Histogram of neuron output values from \nth{8} add layer of ResNet-34. The
    neuron output values resemble a normal distribution, and so nearly all
    neuron output values are contained within the interval \protect$[-2, 2]$.
    This is largely due to the BatchNorm layer preceding the skip connection as
    well as the BatchNorm layer within the non-identity skip branch.%
  }
  \label{fig:layer_histogram}
\end{figure}


==> tikz/strategies/common.tex <==
\newcommand{\flowerpath}{../../img/misc/flower.pdf}

\def\arrowx{2cm}
\def\itemx{1cm}
\def\padx{0.50cm}
\def\widex{1.5cm}

\tikzstyle{item} = [
  minimum width=2*\itemx,
  minimum height=2cm,
]

\tikzstyle{wide} = [
  item,
  minimum width=2*\widex,
]

\tikzstyle{description} = [
  font=\small,
  align=center,
  scale=0.8,
]

\tikzstyle{label} = [
  font=\small\ttfamily,
  scale=0.8,
  green!40!black,
]

\tikzstyle{feedarrow} = [
  -{Latex[length=0.6cm, width=0.8cm]},
  line width=0.30cm,
  draw=orange!50,
]

\tikzstyle{signal} = [
  draw=red!75!blue!85,
  thick,
  smooth,
]

\tikzstyle{signalplot} = [
  domain=0:1,
  samples=50,
]

\tikzset{
    declare function={
      sinf(\t,\f) = sin(deg(2 * pi * \f * \t));
      cosf(\t,\f) = cos(deg(2 * pi * \f * \t));
      modulate(\t) = 0.1 * sinf(\t, 20);
      source(\t) = sinf(\t, 6) * sinf(\t, 3) * sinf(modulate(\t) + \t, 0.88);
      window(\t) = (0.5 - cosf(\t, 1) / 2)^2;
      signal(\t) = source(\t) * window(\t);
    }
}

% [drawopts]{x}{y}{width}{height}{depth}
\newcommand{\cube}[6][]{%
  \draw[#1] ($(#4, #5, 0) + (#2, #3, 0)$)
    -- ++(-#4, 0, 0) -- ++(0, -#5, 0) -- ++(#4, 0, 0) -- cycle;
  \draw[#1] ($(#4, #5, 0) + (#2, #3, 0)$)
    -- ++(0, 0, -#6) -- ++(0, -#5, 0) -- ++(0, 0, #6) -- cycle;
  \draw[#1] ($(#4, #5, 0) + (#2, #3, 0)$)
    -- ++(-#4, 0, 0) -- ++(0, 0, -#6) -- ++(#4, 0, 0) -- cycle;
}

% {x}{channels}{width_and_height}
\newcommand{\layercube}[4][]{%
  %                   {x} {y}    {w} {h} {d}
  \cube[fill=white,#1]{#2}{-#4/2}{#3}{#4}{#4}%
}

